New Additive Spanner Lower Bounds by an Unlayered Obstacle Product

For an input graph $G$, an additive spanner is a sparse subgraph $H$ whose shortest paths match those of $G$ up to small additive error. We prove two new lower bounds in the area of additive spanners: 1) We construct $n$-node graphs $G$ for which any spanner on $O(n)$ edges must increase a pairwise distance by $+\Omega(n^{1/7})$. This improves on a recent lower bound of $+\Omega(n^{1/10.5})$ by Lu, Wein, Vassilevska Williams, and Xu [SODA '22]. 2) A classic result by Coppersmith and Elkin [SODA '05] proves that for any $n$-node graph $G$ and set of $p = O(n^{1/2})$ demand pairs, one can exactly preserve all pairwise distances among demand pairs using a spanner on $O(n)$ edges. They also provided a lower bound construction, establishing that that this range $p = O(n^{1/2})$ cannot be improved. We strengthen this lower bound by proving that, for any constant $k$, this range of $p$ is still unimprovable even if the spanner is allowed $+k$ additive error among the demand pairs. This negatively resolves an open question asked by Coppersmith and Elkin [SODA '05] and again by Cygan, Grandoni, and Kavitha [STACS '13] and Abboud and Bodwin [SODA '16]. At a technical level, our lower bounds are obtained by an improvement to the entire obstacle product framework used to compose "inner" and "outer" graphs into lower bound instances. In particular, we develop a new strategy for analysis that allows certain non-layered graphs to be used in the product, and we use this freedom to design better inner and outer graphs that lead to our new lower bounds.

==> intro_backup.tex <==
\section{Introduction}

In robotics \cite{Cai94}, circuit design \cite{CKRS90, CKRS92, SCRS01}, distributed algorithms \cite{Awerbuch85, BCLR86}, and many other areas of computer science (see survey \cite{ABSHJKS20}), one often wants to compress a graph metric $G$ into small space while approximately preserving its shortest path distances.
When this compression is achieved by a sparse subgraph $H \subseteq G$ whose distance metric is similar to that of $G$, we call $H$ a \emph{spanner} of $G$.
The setting of linear or near-linear size spanners is considered particularly important in applications; that is, for an input graph on $n$ nodes, we often want spanners on $O(n)$ or perhaps $O(n^{1+\eps})$ edges \cite{ABSHJKS20}.

Spanners were first abstracted by Peleg and Upfal \cite{PU89jacm} and Peleg and Ullman \cite{PU89sicomp} after arising implicitly in prior work.
Their initial work studied spanners in the setting of \emph{multiplicative} error:
\begin{definition} [Multiplicative Spanners]
For a graph $G$, a subgraph $H \subseteq G$ over the same vertex set is a $\cdot k$ multiplicative spanner of $G$ if, for all nodes $s, t$, we have $\dist_H(s, t) \le k \cdot \dist_G(s, t)$.
\end{definition}

Optimal bounds for multiplicative spanners were quickly closed in a classic paper by Alth{\" o}fer, Das, Dobkin, Joseph, and Soares \cite{ADDJS93}.
For the specific case of $O(n)$-size spanners, they proved:
%In this exposition we will treat all graphs as undirected and unweighted (even though a few theorems, including the following, extend to the weighted setting).
\begin{theorem} [\cite{ADDJS93}] \label{thm:multspan}
Every $n$-node graph has a $\cdot O(\log n)$ multiplicative spanner on $O(n)$ edges.
This is tight, in the sense that there are graphs that do not have an $\cdot o(\log n)$ multiplicative spanner on $O(n)$ edges.
\end{theorem}
Thus, the question of compression by multiplicative spanners was closed.
However, for many problems, the paradigm of multiplicative error is considered unacceptable.
For example,  $\cdot O(\log n)$ multiplicative blowup in travel time due to compression error would be unacceptable for a cross-country trucking route.
This generated interest in the community in new error paradigms that perform better on the \emph{long} distances in the graph input graph.
Several new types of spanners were suggested and studied in the following years \cite{EP04, TZ06}.
The most optimistic was \emph{purely additive spanners}, where pairwise distances in the spanner increase only by an \emph{additive} term that is independent of the original distance in $G$.
Formally:
\begin{definition} [Additive Spanners \cite{LS91}]
For a graph $G$, a subgraph $H \subseteq G$ over the same vertex set is a $+k$ additive spanner of $G$ if, for all nodes $s, t$, we have $\dist_H(s, t) \le \dist_G(s, t) + k$.
\end{definition}

Unfortunately, high-quality constructions of near-linear-size spanners with purely additive error remained elusive.
That is, the community faced the following question:

\begin{center}
    \emph{Do all graphs admit $+k$ additive spanners of near-linear size, with $k$ a constant, or at least a small enough function of $n$ to be practically efficient?}
\end{center}

This problem became a central focus of the community following a sequence of upper bound results.
First was the seminal 1995 work of Aingworth, Chekuri, Indyk, and Motwani \cite{ACIM99}, which proved that every $n$-node graph has a $+2$ additive spanner on $O(n^{3/2})$ edges.
This was followed by a theorem of Chechik \cite{Chechik13soda} that all graphs have $+4$ spanners on $\Oish(n^{7/5})$ edges (see also \cite{AlDhalaan21}), and from Baswana, Kavitha, Mehlhorn, and Pettie \cite{BKMP10} who proved that all graphs have $+6$ spanners on $O(n^{4/3})$ edges (see also \cite{Woodruff10, Knudsen14}).
Thus, it seemed that one might be able to continue this trend, paying more and more constant additive error in exchange for sparser and sparser spanners.
Unfortunately, a barrier to further progress was discovered by Abboud and Bodwin \cite{AB17jacm}, who constructed graphs for which any additive spanner on $O(n^{4/3 - c})$ edges suffers $+k=n^{\Omega(1)}$ additive error.
Thus, near-linear spanners with subpolynomial error are not generally possible.

At the same time, the lower bound in \cite{AB17jacm} left open the possibility of $O(n)$-size spanners whose (polynomial) additive error term is small enough to be entirely practical.
The lower bound for $O(n)$-size spanners from \cite{AB17jacm} is $+k=n^{1/22}$ additive error, which is reasonable even on enormous input graphs.
However, the upper bounds for $O(n)$-size spanners were far from this ideal.
The first nontrivial constructions of $O(n)$-size spanners \cite{Pettie09} (following \cite{BCE05}) had $+n^{9/16}$ error.
Thus began a focused effort by the community to narrow these upper and lower bounds on additive error towards the middle, with the goal to determine whether practically-significant constructions of near-linear additive spanners can be generally achieved.

Despite a high throughput of recent work on the topic, the attainable error bounds for linear-size additive spanners remain wide open.
The initial lower bound of $n^{1/22}$ additive error was improved to $n^{1/11}$ in two concurrent papers \cite{HP18, Lu19}, and then recently to $n^{1/10.5}$ by Lu, Vassilevska Williams, Wein, and Xu \cite{LVWX22} where it stands today.
Meanwhile, the upper bound on error was improved to $\Oish(n^{1/2})$ \cite{BV15} and then to $n^{3/7 + \eps}$ \cite{BV16} (see also \cite{Chechik13soda, Pettie09}).
This paper further improves the lower bound:
\begin{theorem} [Main Result]
There are $n$-node graphs that do not admit a $+o(n^{1/7})$ additive spanner on $O(n)$ edges.
\end{theorem}


% \begin{center}
%     \begin{tikzpicture}{|lll|}
%     \draw [ultra thick] (0, 0) -- (12, 0);
    
%     %%%%%%%%%%%% LOWER
%     \draw [red] (0, 0) circle [radius=0.15];
%     \node [color=red] at (0, -0.5) {$\Omega(\log n)$ \cite{Woodruff06, girth}};
    
%     \draw [fill=red] ({12/22}, 0) circle [radius=0.15];
%     \node [color=red] at ({12/22}, -0.5) {$\Omega\left(n^{1/22}\right)$ \cite{AB17jacm}};

%     \draw [fill=red] ({12/11}, 0) circle [radius=0.15];
%     \node [color=red] at ({12/11}, -0.5) {$\Omega\left( n^{1/11} \right)$ \cite{HP18, Lu18?}};
    
%     \draw [fill=red] ({12/10.5}, 0) circle [radius=0.15];
%     \node [color=red] at ({12/10.5}, -0.5) {$\Omega\left( n^{1/11} \right)$ \cite{HP18, Lu18?}};
    
%     %%%%%%%%% UPPER
%     \draw [fill=green] (12, 0) circle [radius=0.15];
%     \node [color=green] at (12, -0.5) {$O(n)$ \cite{BCE03}};
    
%     \draw [fill=green] ({12*9/16}, 0) circle [radius=0.15];
%     \node [color=green] at ({12*9/16}, -0.5) {$O\left(n^{9/16}\right)$ \cite{Pettie08}};

%     \draw [fill=green] ({12*1/2}, 0) circle [radius=0.15];
%     \node [color=green] at ({12*1/2}, -0.5) {$\Oish\left(n^{1/2}\right)$ \cite{BV16}};
    
%     \draw [fill=green] ({12*3/7}, 0) circle [radius=0.15];
%     \node [color=green] at ({12*3/7}, -0.5) {$\Oish\left(n^{3/7+\eps}\right)$ \cite{BV16}};
    
%     %%%%%%%%% NEW
%     \draw [fill=red] ({12/7}, 0) circle [radius=0.15];
%     \node [color=red] at ({12/7}, -0.5) {$\Omega\left( n^{1/7} \right)$ \cite{HP18, Lu18?}};
    
%     \draw [fill=white] ({12/3}, 0) circle [radius=0.15];


%     \end{tikzpicture}
% \end{center}

% \grnoteinline{I'm not sure how I feel about this picture currently (besides the overlapping captions lol).  It compresses the lower bounds together in a way that makes their level of technical improvement look smaller than it really is.  Maybe try drawing on a $\log \log$ scale instead?  Also need to add the new upper bound}


% title commands are \section, \subsection, \subsubsection and \paragraph

==> upperbounds.tex <==




\section{Improved Upper Bounds for Spanners and Emulators}

In this section, we present  new constructions for linear-sized additive spanners and emulators. We obtain improved extremal upper bounds on the additive distortion of these two objects via a simple recursive argument. Our construction will make  use of the graph clustering decomposition of \cite{BV16}. We restate the necessary lemma of \cite{BV16} below.

For the remainder of this section, we  use $\widehat{O}(\cdot)$ to hide $n^{O(\epsilon)}$ factors and $O_{\epsilon}(\cdot)$ to hide constant factors dependent on $\epsilon$  in our asymptotic notation. We let $B(v, r)$ denote the set of nodes of distance at most $r$ from $v$ in $G$. 

\begin{lemma}[Lemma 13 of \cite{BV16}] 
\label{lem:clustering_lem}
Let  $r \in [1, n]$ and  $\epsilon > 0$. 
For every $n$-node graph $G = (V, E)$, there exists a set of nodes $\mathcal{C} = \{v_1, \dots, v_k\}$ and corresponding integers $\mathcal{R} = \{r_1, \dots, r_k\}$, where $r_i = \widehat{\Theta}(r)$, satisfying the following:
\begin{itemize}
    \item (Coverage) For each $v \in V$, $v \in B(v_i, r_i)$ for some $i \in [1, k]$.  
    \item (Low Overlap) $\sum_{i=1}^k|B(v_i, 2r_i)| = O_{\epsilon}(n)$.
\end{itemize}
\end{lemma}
For $i \in [1, k]$, we will think of set $B(v_i, 2r_i)$ as a cluster of vertices in $G$, and we will refer to $B(v_i, r_i)$ as the core of cluster $B(v_i, 2r_i)$. Note that the coverage property of Lemma \ref{lem:clustering_lem} states that every vertex in $V$ belongs to the core of some cluster in the  decomposition. For every vertex $v$ in $V$, we let $C(v)$ denote a cluster $B(v_i, 2r_i)$ containing $v$ in its core. 


The basic idea for our spanner and emulator upper bounds will be the same. In the preprocessing phase, we will choose a radius $r$ and perform the above cluster decomposition. For each $v_i \in \mathcal{C}$, we define a corresponding cluster $B(v_i, 2r_i)$. We then categorize our clusters as either being \textit{small} or \textit{large}, based on the number of nodes in the cluster. In small clusters, we will preserve the distances between vertices exactly, using a simple sampling scheme. In  large clusters, we will recursively insert a linear-sized spanner (or emulator) over the cluster to approximately preserve distances. This will complete the preprocessing phase. 
We then add the rest of the edges to our spanner (or emulator) in a greedy fashion similar to previous additive spanner constructions  \cite{BKMP10, BV16, Knudsen14}.




\section{Improved Emulator Upper Bound}
For expository purposes, we begin by presenting our emulator upper bound, which has a simpler analysis than the spanner upper bound. In our construction, we will recursively use old emulator upper bounds to obtain new and improved emulator upper bounds. This is formalized in the following lemma.


\begin{lemma}
Suppose for every $n$-node graph $G$ and every $\epsilon > 0$ there exists an additive emulator of $G$ with $O_{\epsilon}(n)$ edges and distortion $+O(n^{\alpha + \epsilon})$, where $\alpha \in (0, 1)$. Then for every $n$-node graph $G$ and every $\epsilon > 0$ there exists an additive emulator of $G$ with $O_{\epsilon}(n)$ edges and distortion $+O(n^{1/(6-4\alpha) + \epsilon })$. 
\label{lem:emu_recursion}
\end{lemma}

\begin{proof} Let $H$ denote our new emulator of $G$. We first give the construction of $H$, and then we prove that $H$ has our desired properties.

\paragraph{Construction.}  Begin the preprocessing phase by adding a linear-sized multiplicative spanner with $\cdot \log n$ distortion to $H$. Let $r = n^{1/(6 - 4 \alpha)}$.  Sample each $v \in V$ into $V'$ independently with probability $\Theta(r^{-1} \log n)$. Now perform the clustering decomposition of Lemma \ref{lem:clustering_lem} with parameters $r$ and  $\epsilon > 0$ to obtain a set of cluster centers $\mathcal{C} = \{v_1, \dots, v_k\}$ and corresponding cluster radii $\mathcal{R} = \{r_1, \dots, r_k\}$. By Lemma \ref{lem:clustering_lem},  there exists a universal constant $c > 0$  such that  $2r_i \log n \leq r\cdot n^{c\epsilon}$ for $i \in [1, k]$. We let $\hat{r}$ denote $r\cdot n^{c\epsilon}$. 

Fix an $i \in [1, k]$. We say that $B(v_i, 2r_i)$ is a \textit{small} cluster if $|B(v_i, 2r_i)| \leq  r^{2}\log^{-2}n$. Else we say that $B(v_i, 2r_i)$ is a \textit{large} cluster. If $B(v_i, 2r_i)$ is a small cluster, then for all  vertices $s, t$ in $B(v_i, 2r_i) \cap V'$, add the emulator edge $(s, t)$ with weight $d_G(s, t)$ to $H$.
If $B(v_i, 2r_i)$ is a large cluster, then we recursively call our presupposed emulator procedure on the induced subgraph $G' = G[B(v_i, 2r_i)]$ with parameter $\epsilon$ to obtain a emulator $H'$ with $O_{\epsilon}(|B(v_i, 2r_i)|)$ edges and additive distortion $+O(|B(v_i, 2r_i)|^{\alpha + \epsilon})$. We add the edges of $H'$ to $H$.
By repeating the previous steps for all $i \in [1, k]$ we complete the preprocessing phase.

Now we greedily add emulator edges to $H$ to connect the remaining pairs of vertices violating our spanner property. 
While there exists vertices $s, t$ in $V$ such that $d_H(s, t) > d_G(s, t) + 16\hat{r}$, do the following. Let $\pi$ be a shortest $(s, t)$-path. Let $x$ be the vertex in $\pi$ farthest from $s$ such that
for any two vertices $u, w$ in $ \pi(s, x)$, $d_H(u, w) \leq d_G(u, w) + \hat{r}$. Additionally,  let $y$ be the vertex in $\pi$ farthest from $t$ such that for any two vertices $u, w$ in $\pi(y, t)$,   $d_H( u, w) \leq d_G(u, w) + \hat{r}$. Add emulator edge $(x, y)$ with weight $d_G(x, y)$ to $H$. This greedy phase completes the construction. Our procedure is summarized in Figure \ref{fig:new_emulator}. 

\begin{figure}[h]
    \centering


\fbox{
\begin{minipage}[c]{0.9\textwidth}
\begin{center}
    \textbf{Additive Emulator Procedure} \texttt{NewEmulator}:
\end{center}
\textbf{Input:}
\begin{itemize}
    \item An $n$-node graph $G = (V, E)$ and a parameter $\epsilon > 0$.
    \item A procedure \texttt{OldEmulator}, which takes as input a graph $G'$, and outputs an additive emulator $H'$ of $G'$ with   $O_{\epsilon}(|G'|)$ edges and distortion $+O(|G'|^{\alpha + \epsilon})$. 
\end{itemize}
    \textbf{Output:} An additive emulator $H$ of $G$ with $O_{\epsilon}(n)$ edges and distortion $+\widehat{O}(n^{1/(6 - 4  \alpha ) })$. 
\\

\textbf{Preprocessing Phase:}
\begin{enumerate}
    \item Add a linear-sized spanner with $\cdot \log n$ multiplicative distortion to $H$.
    \item Let $r = n^{1/(6 - 4 \alpha )}$. Sample each vertex $v \in V$ into $V'$ independently with probability $\Theta(\log n / r)$. 
    \item Perform the clustering decomposition of Lemma \ref{lem:clustering_lem} with parameters $r$ and $\epsilon$ to obtain a set of cluster centers $\mathcal{C} = \{v_1, \dots, v_k\}$ and corresponding cluster radii $\mathcal{R} = \{r_1, \dots, r_k\}$. Let $\hat{r} = r \cdot n^{c\epsilon}$ for a sufficiently large universal constant $c$.
    \item Fix an $i \in [1, k]$. If $|B(v_i,  2r_i)| \leq r^2 \log^{-2} n$, then for all vertices $s, t$ in $B(v_i, 2r_i) \cap V'$, add  edge $(s, t)$ with weight $d_G(s, t)$ to $H$.
    \item Else if $|B(v_i, 2r_i)| > r^{2}\log^{-2}n$, then call \texttt{OldEmulator} on graph $G[B(v_i, 2r_i)]$. Add the emulator output by \texttt{OldEmulator} to $H$.  Repeat steps 4 and 5 for all $i \in [1, k]$. 
\end{enumerate}
\textbf{Greedy Phase:}

While there exist vertices $s, t$ in $V$ such that $d_H(s, t) > d_G(s, t) + 16\hat{r}$, do the following. Let $\pi$ be a shortest $(s, t)$-path. 
Let $x$ be the vertex in $\pi$ farthest from $s$ such that
for any two vertices $u, w$ in $ \pi(s, x)$, $d_H(u, w) \leq d_G(u, w) + \hat{r}$. Additionally,  let $y$ be the vertex in $\pi$ farthest from $t$ such that for any two vertices $u, w$ in $\pi(y, t)$,   $d_H( u, w) \leq d_G(u, w) + \hat{r}$. Add edge $(x, y)$  with weight $d_G(x, y)$ to $H$. 
\end{minipage}
}
    \caption{The recursive procedure for the improved emulator upper bounds. }
    
    \label{fig:new_emulator}
\end{figure}


\paragraph{Bounding the distortion.}  Fix  vertices $s, t \in V$.  If $d_H(s, t) \leq d_G(s, t) + 16\hat{r}$, then we are done. Otherwise, vertex pair $(s, t)$ is considered in some round of the greedy phase. Let path $\pi$ and vertices $x, y$ be as defined in the construction. Note that since edge $(x, y)$ is in $H$, $d_H(x, y) = d_G(x, y)$. 
We have the following:
\begin{align*}
    d_H(s, t) & \leq d_H(s, x) + d_H(x, y) + d_H(y, t) \\ 
   & \leq (d_G(s, x) + \hat{r}) + d_G(x, y) + d_G(y, t) + \hat{r}) \\
 &   \leq d_G(s, t) + 2\hat{r}
\end{align*}
Since $\hat{r} = r \cdot n^{c\epsilon}$ for a universal constant $c > 0$, we may obtain our desired distortion  by taking our construction parameter $\epsilon > 0$ to be sufficiently small.

\paragraph{Bounding the size.} We begin by bounding the number of edges added to $H$ in the preprocessing phase.  Fix an $i \in [1, k]$. If $B(v_i, 2r_i)$ is a small cluster, then with high probability $|B(v_i, 2r_i) \cap V'| = O(r \log^{-1} n)$. Since we add an emulator edge between every pair of vertices in $B(v_i, 2r_i) \cap V'$, it follows that we add at most $|B(v_i, 2r_i) \cap V'|^2 = O(|B(v_i, 2r_i)|)$ edges to $H$. Otherwise, if $B(v_i, 2r_i)$ is a large cluster, then our recursive emulator call contributes $O_{\epsilon}(|B(v_i, 2r_i)|)$ edges to $H$. Then by the low overlap property of Lemma \ref{lem:clustering_lem}, we add $O_{\epsilon}(n)$ edges to $H$ in the preprocessing phase. 


To bound the number of edges added in the greedy phase, we use a path buying argument reminiscent of the proof in \cite{BV16}. We say that vertices $s, t$ in $V$ are \textit{connected} in $H$ if $d_H(s, t) \leq d_G(s, t) + 8\hat{r}$. Each time we add an emulator edge to $H$ in the greedy phase, we will argue that $\Omega(n)$ pairs of vertices in $V$ become connected in $H$ for the first time. Then since there are $O(n^2)$ pairs of vertices in $V$, the greedy phase adds $O(n)$ edges to $H$. 

Let $(s, t)$ be a pair of vertices considered in some round of the greedy phase. Let path $\pi$ and vertices $x, y$ be as defined in the construction. We say that paths $\pi(s, x)$ and $\pi(y, t)$ are the prefix and suffix of $\pi$, respectively. We will define a set $S$ of vertices in $G$ near the prefix of $\pi$ and a set $T$ of vertices in $G$ near the suffix of $\pi$. Then we will show that after adding edge $(x, y)$ to $H$,  all pairs of vertices in $S \times T$ become connected in $H$ for the first time. Finally, we will establish that $|S \times T| = \Omega(n)$, completing the proof.

We define $S$ and $T$ as follows:
\[
S := \cup_{v \in \pi(s, x)} C(v) \qquad \text{ and } \qquad T := \cup_{v \in \pi(y, t)} C(v).
\]
We now verify that $S$ and $T$ satisfy our desired properties.


%  We now explicitly construct $S$. Starting at $s$, let $s_1$ be a vertex in $\pi(s, x) \cap V'$ such that $d_G(s, s_1) \leq r$. Add the vertices in $C(s_1)$ to $S$. Now let $s_2$ be a vertex in $\pi(s_1, x) \cap V'$ such that $r/2 \leq d_G(s_1, s_2) \leq r$, and add $C(s_2)$ to $S$.  More generally, we let $s_{i+1}$ be a vertex in $\pi(s_i, x) \cap V'$ such that $r/2 \leq d_G(s_i, s_{i+1}) \leq r$, and we add $C(s_i)$ to $S$.
%  Since we sample each vertex in $V$ into $V'$ with probability $\Theta(\log n / r)$, we will always be able to find the next vertex $s_i$ satisfying the above criteria with high probability by the  Chernoff bound and the union bound. 
%  We repeat this procedure until we obtain a maximal set $S' := s_1, s_2, \dots, s_{\ell}$ such that $d_H(s_i, s_j) \leq d_G(s_i, s_j) + \hat{r}/2$ for $i, j \in [1, \ell]$. Note that we define $S$ to be $S := \cup_{s_i \in S'} C(s_i)$. 


% We now define $S$ and $T$. Let $S' := s_1, s_2, \dots, s_{\ell}$ be a maximal set of vertices in $\pi(s, x) \cap V'$ satisfying the following conditions: 
% \begin{enumerate}
%     \item $d_G(s, s_i) < d_G(s, s_j)$ for $i < j \in [1, \ell]$
%     \item $d_G(s, s_1) \leq r$
%     \item $r/2 \leq d_G(s_i, s_{i+1}) \leq r$ for $i \in [1, \ell - 1]$
%     \item $d_H(s_i, s_j) \leq d_G(s_i, s_j) + \hat{r}/2$ for $i, j \in [1, \ell ]$. 
% \end{enumerate}
% Note that by condition 1, vertices $s_1, \dots, s_{\ell}$ are listed in the order they appear in $\pi(s, x)$.  Additionally, note that since we sample each vertex in $V$ into $V'$ with probability $\Theta(\log n / r)$, conditions 2 and 3 are true with high probability by the Chernoff bound and the union bound. Consequently, only condition 4 imposes a  constraint on the size of $S'$. 
% We let $S := \cup_{s_i \in S'} C(s_i)$. We define $T$ symmetrically. Let $T' := t_1, t_2, \dots, t_{\ell'}$ be a maximal set of vertices in $\pi(y, t)$ satisfying the following conditions:
% \begin{enumerate}
%     \item $d_G(t, t_i) < d_G(t, t_j)$ for $i < j \in [1, \ell']$
%     \item $d_G(t, t_1) \leq r$
%     \item $r/2 \leq d_G(t_i, t_{i+1}) \leq r$ for $i \in [1, \ell' - 1]$
%     \item $d_H(t_i, t_j) \leq d_G(t_i, t_j) + \hat{r}/2$ for $i, j \in [1, \ell']$,
% \end{enumerate}
% and let $T := \cup_{t_i \in T'} C(t_i)$. We now claim that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$, and $\pi(t_{\ell'}, t)$ is a subpath of $\pi(y, t)$. Let $u, w$ be vertices in $\pi(s, s_{\ell})$. Suppose that $u$ occurs before $w$ in $\pi(s, s_{\ell})$. Let $s_i$ be the vertex in $\pi(u, w) \cap \{s_1, s_2, \dots, s_{\ell}\}$ closest to $u$, and let $s_j$ be the vertex in $\pi(u, w) \cap \{s_1, s_2, \dots, s_{\ell}\}$ closest to $w$. Then observe the following:
% \begin{align*}
%     d_H(u, w) & \leq d_H(u, s_i) + d_H(s_i, s_j) + d_H(s_j, w) \\
%     & \leq \log n \cdot d_G(u, s_i) + d_H(s_i, s_j) + \log n \cdot d_G(s_j, w) \\
%     & \leq d_G(u, s_i) +  d_H(s_i, s_j) + d_G(s_j, w) + 2r\log n  \\
%     & \leq d_G(u, s_i) + d_G(s_i, s_j) + d_G(s_j, w) + \hat{r}/2 + 2r\log n \\
%     & \leq d_G(u, w) + \hat{r}.
% \end{align*}
% The second inequality follows from the insertion of a $\cdot \log n$ multiplicative spanner in $H$, and the final inequality follows from the fact that $\pi(u, w)$ is a $(u, w)$-shortest path in $G$ and $\hat{r} = r\cdot n^{c\epsilon}$. 
% Then by our choice of $x$, we conclude that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$. An identical argument shows that $\pi(t_{\ell'}, t)$ is a subpath of $\pi(y, t)$. We now verify that $S \times T$ has our desired property.



% % Let $U = u_1, u_2, \dots, u_{\ell}$ be the vertices in $\pi \cap V'$, listed in the order they appear in $\pi$. We define our sets $S$ and $T$ to be 
% % \[
% % S = \cup_{u_i \in \pi(s, x) \cap U} C(u_i) \text{ and } T = \cup_{u_i \in \pi(y, t) \cap U} C(u_i)
% % \]
% % So $S$ contains  vertices in the clusters near the prefix $\pi(s, x)$ of $\pi$, and $T$ contains  vertices in the clusters near the suffix $\pi(y, t)$ of $\pi$. 

\begin{proposition}
After edge $(x, y)$ is added to $H$, all pairs of vertices in $S \times T$ become connected in $H$ for the first time.
\label{prop:first_conn}
\end{proposition}
\begin{proof}
Note that every vertex in $S$ or $T$ is within distance $\hat{r} \log^{-1} n$ of some vertex in $\pi(s, x)$ or $\pi(y, t)$, respectively, in $G$.  Fix vertices $s' \in S$ and $t' \in T$, and let $x'$  (respectively, $y'$) be the vertex in $\pi(s, x)$ (respectively,  $\pi(y, t)$) that is closest to $s'$ (respectively,  $t'$) in $G$.
 (See Figure \ref{fig:emulator_pic} for a visualization.)
After edge $(x, y)$ is added to $H$, $s'$ and $t'$ are connected in $H$:
\begin{align*}
d_H(s', t')  & \leq d_H(s', x') + d_H(x', y') + d_H(y', t') \\
& \leq \log n \cdot d_G(s', x') + d_H(x', y') + \log n \cdot d_G(y', t')  \\
& \leq \hat{r} + d_H(x', x) + d_H(x, y) + d_H(y, y') + \hat{r} \\
& \leq  (d_G(x', x) + \hat{r}) + d_G(x, y) + (d_G(y, y') + \hat{r}) +2\hat{r} \\
& \leq  d_G(x', y')  + 4\hat{r} \\
& \leq d_G(x', s') + d_G(s', t') + d_G(t', y') + 4\hat{r} \\
& \leq d_G(s', t') + 6\hat{r},
\end{align*}
where the second inequality follows from the $\cdot \log n$ multiplicative spanner in $H$, and the fifth inequality follows from the fact that $\pi(x', y')$ is a shortest path in $G$.  Now suppose for the sake of contradiction that $s'$ and $t'$ were connected in $H$ \textit{before} edge $(x, y)$ is added to $H$. Then we claim that pair $(s, t)$ had low distortion in $H$ before edge $(x, y)$ was added: 
\begin{align*}
    d_H(s, t) & \leq d_H(s, x') + d_H(x', y') + d_H(y', t) \\
    & \leq d_G(s, x') + d_H(x', s') + d_H(s', t') + d_H(t', y') + d_G(y', t) + 2\hat{r} \\
    & \leq d_G(s, x') + \log n \cdot d_G(x', s') + d_H(s', t') + \log n \cdot d_G(t', y') + d_G(y', t) + 2\hat{r} \\
    & \leq d_G(s, x') + d_H(s', t') + d_G(y', t) + 4\hat{r} \\
    & \leq d_G(s, x') + (d_G(s', t') + 8\hat{r}) + d_G(y', t) + 4\hat{r} \\
    & \leq d_G(s, x') + (d_G(s', x') + d_G(x', y') + d_G(y', t')) + d_G(y', t) + 12\hat{r} \\
    & \leq d_G(s, x') + d_G(x', y') + d_G(y', t) + 14\hat{r} \\
    & \leq d_G(s, t) + 14\hat{r}
\end{align*}
This contradicts our assumption that pair $(s, t)$ was considered in this round of the greedy phase. We conclude that all pairs of vertices in $S \times T$ are connected for the first time after edge $(x, y)$ is added to $H$.
\end{proof}

\begin{figure}[h]
    \centering
    \includegraphics{emulator_draw.pdf}
    \caption{The solid black line denotes path $\pi$ in $G$. After edge $(x, y)$ is added to $H$ in the greedy phase, all pairs of vertices  $(s', t')$ in $S \times T$ become connected in $H$ for the first time. }
    \label{fig:emulator_pic}
\end{figure}


% Let $S = \cup_{i=1}^{\ell} C(u_i)$. We define set $T$ symmetrically. Namely, let $T = $

What remains is to show that $|S \times T| = \Omega(n)$. Specifically, we will show that $|S| = \Omega(n^{1/2})$, and $|T| = \Omega(n^{1/2})$ will follow by a symmetric argument. Notice that the size of $S$ is constrained by our requirement that for any two vertices $u, w$ in $\pi(s, x)$, $d_H(u, w) \leq d_G(u, w) + \hat{r}$. 
\begin{proposition}
$|S \times T| = \Omega(n)$
\label{prop:s_t_size}
\end{proposition}
\begin{proof}
Instead of lower bounding $|S|$ directly, we  find it easier to lower bound a subset $S' \subseteq S$. We now explicitly construct $S'$. We begin the construction by initializing two sets as $U := \emptyset$ and $S' := \emptyset$ and setting an integer counter 
$\texttt{err} := 0$. Starting at $s$, we walk through $\pi(s, x)$ as follows. Let $s_1$ be a vertex in $\pi(s, x) \cap V'$ such that $d_G(s, s_1) \leq r$. Note that since we sample vertices in $V$ into $V'$ with probability $\Theta(\log n / r)$, such a vertex $s_1$ will exist with high probability by the Chernoff bound. Add $s_1$ to $U$ and add the vertices in $C(s_1)$ to $S'$. Now, given $s_i$, we let $s_{i+1}$ be a vertex in $\pi(s_i, x) \cap V'$ such that $r/2 \leq d_G(s_i, s_{i+1}) \leq r$. Again by the Chernoff bound, such a vertex $s_{i+1}$ will exist with high probability.
Add vertex $s_{i+1}$ to $U$, and add the vertices in cluster $C(s_{i+1})$ to $S'$. 
If $C(s_i)$ is a large cluster, then we increment $\texttt{err}$ by $+O(|C(s_i)|^{\alpha + \epsilon})$, which corresponds to the distortion of the linear sized emulator of $C(s_i)$ we inserted into $H$ in the preprocessing phase. We proceed in this manner until we add the first vertex $s_{\ell}$ such that $\texttt{err} + O(|C(s_{\ell})|^{\alpha + \epsilon}) > \hat{r} / 2$. (This implies that  $\texttt{err} \leq \hat{r} /2$.) Note that $S' = \cup_{s_i \in U}C(s_i)$.

Now we verify that $S' \subseteq S$, as desired. To prove this, it will suffice to show that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$. Fix an $i \in [1, \ell - 1]$ and suppose that $C(s_i)$ is a small cluster. Then since $s_i$ is in the core of cluster $C(s_i)$ and $d_G(s_i, s_{i+1}) \leq r$, it follows that $s_{i+1} \in C(s_i)$.  Note that in this case, emulator edge $(s_i, s_{i+1})$ is added to $H$ in the preprocessing phase, allowing us to travel from $s_i$ to $s_{i+1}$ without incurring any error. Specifically, $d_H(s_i, s_{i+1}) = d_G(s_i, s_{i+1})$.  Otherwise, $C(s_i)$ is a large cluster. In this case, we added an emulator of $G[C(s_i)]$ with additive distortion $+O(|C(s_i)|^{\alpha + \epsilon})$ to $H$ in the preprocessing phase. Note that since $s_i$ is in the core of $C(s_i)$ and $d_G(s_i, s_{i+1}) \leq r$, it follows that any shortest $(s_i, s_{i+1})$-path in $G$ is contained in $G[C(s_i)]$. Consequently, $d_H(s_i, s_{i+1}) \leq d_G(s_i, s_{i+1}) + O(|C(s_i)|^{\alpha + \epsilon})$.
Then by the previous observations, we  conclude that $d_H(s_i, s_j) \leq d_G(s_i, s_j) + \texttt{err}$ for all $i, j \in [1, \ell]$. 
Now let $u, w$ be vertices in $\pi(s, s_{\ell})$ (where $u$ occurs before $w$ in $\pi(s, s_{\ell})$), and let $s_i, s_j$ be the vertices in $\pi(s, s_{\ell}) \cap U$ that are closest to  $u$ and closest to $w$, respectively. Observe that
\begin{align*}
    d_H(u, w) & \leq d_H(u, s_i) + d_H(s_i, s_j) + d_H(s_j, w) \\
    & \leq \log n \cdot d_G(u, s_i) + d_H(s_i, s_j) + \log n \cdot d_G(s_j, w) \\
    & \leq d_G(u, s_i) + d_H(s_i, s_j) + d_G(s_j, w) + 2r\log n \\
    & \leq d_G(u, s_i) + (d_G(s_i, s_j) + \texttt{err}) + d_G(s_j, w) + 2r\log n \\
    & \leq d_G(u, w) + \hat{r}/2 + 2r \log n \\
    & \leq d_G(u, w) + \hat{r}.
\end{align*}
Then by our choice of $x$, it follows that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$, so $S' \subseteq S$. 

By our construction of $S'$, we have the guarantee that $\sum_{i=1}^{\ell} O(|C(s_{i})|^{\alpha + \epsilon}) > \hat{r} / 2$. 
Moreover, we may assume that all clusters $C(s_i)$ are  large clusters, since as noted earlier we can travel through small clusters with zero distortion. This implies that $|C(s_i)| \geq r^2 \log^{-2} n$. 
Now we wish to lower bound the sum $\sum_{i=1}^{\ell} |C(s_i)|$. We may assume that $\alpha + \epsilon < 1$, and so by a convexity argument it can be seen that the sum $\sum_{i=1}^{\ell} |C(s_i)|$ is minimized (while subject to our guaranteed  inequality) when each large cluster has size $r^2 \log^{-2}n$. Let $q$ be the number of large clusters we pass through in $\pi(s, s_{\ell})$.  Then our guarantee becomes  $\sum_{i=1}^{\ell} O(|C(s_{i})|^{\alpha + \epsilon}) = q \cdot (r^2 \log^{-2}n)^{\alpha + \epsilon} > \hat{r} / 2$. Rearranging this inequality gives us that $q > \hat{r} \cdot r^{-2(\alpha + \epsilon)}$. Now note that since $\hat{r} = r \cdot n^{c\epsilon}$ for a sufficiently large constant $c$, we may assume that $\hat{r} \geq r^{1 + 2\epsilon} \log^2 n$ by taking $c > 2$. Now putting it all together, we see that
\[
\sum_{i=1}^{\ell}|C(s_i)| \geq q \cdot r^2 \log^{-2} n \geq \frac{\hat{r} \cdot r^2}{r^{2(\alpha + \epsilon)} \cdot \log^2 n} \geq r^{3 - 2\alpha} = n^{(3 - 2\alpha)/(6 - 4\alpha)} = \Theta(n^{1/2}),
\]
where the second to last equality follows from our choice of $r = n^{1/(6 - 4\alpha)}$. 

Now we finish the proof by showing that $|S'| = |\cup_{i=1}^{\ell} C(s_i)| = \Omega(\sum_{i=1}^{\ell}|C(s_i)|)$. Recall that $d_G(s_i, s_{i+1}) \geq r/2$. Then each vertex $v \in V$ can only occur in $O(1)$ distinct clusters $C(s_i)$, where $s_i \in U$, or else we contradict our assumption that $\pi(s, x)$ is a shortest path in $G$. We conclude that $|\cup_{i=1}^{\ell} C(s_i)| = \Omega(\sum_{i=1}^{\ell}|C(s_i)|)$, so $|S| \geq |S'| = \Omega(n^{1/2})$. A symmetric argument shows that $|T| = \Omega(n^{1/2})$, so it follows that $|S \times T| = \Omega(n)$. 
% By the coverage property of Lemma \ref{lem:clustering_lem}, we know that every vertex $u_j$ belongs to some cluster core $B(v_{i_j}, r_{i_j})$ for some $i_j \in [1, k]$. Consequently, $u_{j+1} \in B(v_{i_j}, 2r_{i_j})$. In other words,
% consecutive sampled vertices $u_j, u_{j+1}$  in $\pi$ belong to the same cluster $B(v_{i_j}, 2r_{i_j})$.  
% Fix a $j \in [1, \ell - 1]$. 
% If $B(v_{i_j}, 2r_{i_j})$ is a small cluster, then edge $(u_j, u_{j+1})$ is added to $H$ in the preprocessing phase of the construction, allowing us to travel from $u_j$ to $u_{j+1}$ in $H$  without incurring any error. Otherwise, $B(v_{i_j}, 2r_{i_j})$ is a large cluster.  Then we added an emulator of $G[B(v_{i_j}, 2r_{i_j})]$ with additive distortion $+O(|B(v_{i_j}, 2r_{i_j})|^{\alpha + \epsilon})$ to $H$ in the preprocessing phase. Note that since $u_j \in B(v_{i_j}, r_{i_j})$ and $d_G(u_j, u_{j+1}) \leq r$, it follows that any shortest $(u_j, u_{j+1})$-path is contained in $G[B(v_{i_j}, 2r_{i_j})]$. Consequently, $d_H(u_j, u_{j+1}) \leq d_G(u_j, u_{j+1}) +O(|B(v_{i_j}, 2r_{i_j})|^{\alpha + \epsilon})$. Thus we are able to travel from $u_j$ to $u_{j+1}$ in $H$ while incurring a small amount of error proportional to the size of the cluster $B(v_{i_j}, 2r_{i_j})$.  
% We will use the observations in the previous paragraph to verify that $|S| = \Omega(n^{1/2})$. The size of $S$ is constrained by our requirement that for any two vertices $v, w$ in $\pi(s, x)$, $d_H(v, w) \leq d_G(v, w) + \hat{r}$. Let $U' \subseteq U$ be the vertices $u_i$ in $\pi(s, x) \cap U$  such that $C(u_i)$ is a large cluster. Ignoring the 
% To lower bound $|S|$, it will suffice to lower bound $| \cup_{u_i \in U'} C(u_i)|$. 
\end{proof}
By our path buying argument, we add $O(n)$ emulator edges to $H$ in the greedy phase, so the total size of $H$ is $O_{\epsilon}(n)$. 
In our construction we made use of the Chernoff bound only polynomially many times, so by the union bound our construction succeeds with high probability.  
\end{proof}






Now we can repeatedly apply Lemma \ref{lem:emu_recursion} to obtain a sequence of improved emulator upper bounds. We choose our initial emulator to be the additive emulator implicit in  \cite{Pettie09} with distortion $+O(n^{1/4})$ and  $O(n)$ edges. Then after one application of Lemma \ref{lem:emu_recursion}, we obtain an additive emulator with $O_{\epsilon}(n)$ edges and distortion $+O(n^{1/(6 - 1) + \epsilon}) = +O(n^{1/5 + \epsilon})$. More generally, after $i$ applications of Lemma \ref{lem:emu_recursion}, we obtain an additive emulator with $O_{\epsilon}(n)$ edges and distortion $+O(n^{a_i + \epsilon})$, where $a_i$ is defined by the recurrence relation $a_0 = 1/4$, $a_{i+1} = 1/(6-4a_i)$. The value of $a_i$ converges quickly to the fixed point $\frac{1}{3 + \sqrt{5}} \approx 0.191$. 



\begin{theorem}
For every $n$-node graph $G = (V, E)$ and $\epsilon > 0$, there exists an emulator $H = (V, E')$ on $O_{\epsilon}(n)$ edges with distortion $+O(n^{\frac{1}{3 + \sqrt{5}}+ \epsilon})$. 
\end{theorem}




\section{Improved Spanner Upper Bound}
The spanner upper bound will have the same structure as the emulator upper bound, with only the implementation details differing between them. We begin by proving the following recursive lemma. 

\label{sec:spanner_bound}

\begin{lemma}
Suppose for every $n$-node graph $G$ and every $\epsilon > 0$ there exists an additive spanner of $G$ with $O_{\epsilon}(n)$ edges and distortion $+O(n^{\alpha + \epsilon})$, where $\alpha \in (0, 1)$. Then for every $n$-node graph $G$ and every $\epsilon > 0$ there exists an additive emulator of $G$ with $O_{\epsilon}(n)$ edges and distortion $+O(n^{1/(3 - 4/3 \cdot \alpha ) + \epsilon})$.
\label{lem:spanner_rec}
\end{lemma}

\begin{proof}
Let $H$ denote our new spanner of $G$. We first give the construction of $H$, and then we prove that $H$ has our desired properties.


\paragraph{Construction.} 
Begin the preprocessing phase by adding a linear-sized multiplicative spanner with $\cdot \log n$ distortion to $H$. Let  $r = n^{1/(3 - 4/3 \cdot \alpha)}$.  Sample each $v \in V$ into $V'$ independently with probability $\Theta(r^{-1} \log n)$. Now perform the clustering decomposition of Lemma \ref{lem:clustering_lem} with parameters $r$ and $\epsilon > 0$ to obtain a set of cluster centers $\mathcal{C} = \{v_1, \dots, v_k\}$ and corresponding cluster radii $\mathcal{R} = \{r_1, \dots, r_k\}$.  By Lemma \ref{lem:clustering_lem}, there exists a universal constant $c>0$ such that $2r_i \log n \leq r \cdot n^{c\epsilon}$ for $i \in [1, k]$. We let $\hat{r}$ denote $r \cdot n^{c\epsilon}$. 


\indent Fix an $i \in [1, k]$. We say that $B(v_i, 2r_i)$ is a \textit{small} cluster if $|B(v_i, 2r_i)| \leq r^{4/3} \log^{-2} n$. Else we say that $B(v_i, 2r_i)$ is a \textit{large} cluster. If $B(v_i, 2r_i)$ is a small cluster, then for every $s \in B(v_i, r_i) \cap V'$ and $t \in B(v_i, 2r_i) \cap V'$ such that $d_G(s, t) \leq r$, add a shortest $(s, t)$-path to $H$. We may assume that the collection of paths added to $H$ in this manner is \textit{consistent}, meaning that any two paths intersect at a single contiguous (possibly empty) subpath.  If $B(v_i, 2r_i)$ is a large cluster, then we recursively call our presupposed spanner procedure on the induced subgraph $G' = G[B(v_i, 2r_i)]$ with parameter $\epsilon$ to obtain a spanner $H'$ with $O_{\epsilon}(|B(v_i, 2r_i)|)$ edges and additive distortion $+O(|B(v_i, 2r_i)|^{\alpha + \epsilon})$. We add the edges of $H'$ to $H$. By repeating the previous steps for all $ i \in [1, k]$ we complete the preprocessing phase. 

\indent Now we greedily add edges to $H$ to connect the remaining pairs of vertices violating our spanner property. While there exists vertices $s, t$ in $V$ such that $d_H(s, t) > d_G(s, t) + 32\hat{r}$, do the following.  Let $\pi$ be a shortest $(s, t)$-path.  Let $x$ be the vertex in $\pi$ farthest from $s$ such that
for any two vertices $u, w$ in $ \pi(s, x)$, $d_H(u, w) \leq d_G(u, w) + \hat{r}$. Additionally,  let $y$ be the vertex in $\pi$ farthest from $t$ such that for any two vertices $u, w$ in $\pi(y, t)$,   $d_H( u, w) \leq d_G(u, w) + \hat{r}$. Add a \textit{consistent} shortest $(x, y)$-path to $H$. This completes the construction. Our procedure is summarized in Figure \ref{fig:spanner_upper}. 


\begin{figure}[h]
    \centering

\fbox{
\begin{minipage}[c]{0.9\textwidth}
\begin{center}
    \textbf{Additive Spanner Procedure} \texttt{NewSpanner}:
\end{center}
\textbf{Input:}
\begin{itemize}
    \item An $n$-node graph $G = (V, E)$ and a parameter $\epsilon > 0$.
    \item A procedure \texttt{OldSpanner}, which takes as input a graph $G'$, and outputs an additive spanner $H'$ of $G'$ with   $O_{\epsilon}(|G'|)$ edges and distortion $+O(|G'|^{\alpha + \epsilon})$. 
\end{itemize}
    \textbf{Output:} An additive spanner $H$ of $G$ with $O_{\epsilon}(n)$ edges and distortion $+\widehat{O}(n^{1/(3 - 4/3 \cdot \alpha )})$. 
\\

\textbf{Preprocessing Phase:}
\begin{enumerate}
   \item Add a linear-sized spanner with $\cdot \log n$ multiplicative distortion to $H$.
    \item Let $r = n^{1/(3 - 4/3 \cdot \alpha )}$. Sample each vertex $v \in V$ into $V'$ independently with probability $\Theta(\log n / r)$. 
    \item Perform the clustering decomposition of Lemma \ref{lem:clustering_lem} with parameters $r$ and $\epsilon$ to obtain a set of cluster centers $\mathcal{C} = \{v_1, \dots, v_k\}$ and corresponding cluster radii $\mathcal{R} = \{r_1, \dots, r_k\}$. Let $\hat{r} = r \cdot n^{c\epsilon}$ for a sufficiently large universal constant $c$.
    \item Fix an $i \in [1, k]$. If $|B(v_i, 2r_i)| \leq r^{4/3}\log^{-2}n$, then for all $s \in B(v_i, r_i) \cap V'$ and all $t \in B(v_i, 2r_i) \cap V'$, add a shortest $(s, t)$-path to $H$.
    \item Else if $|B(v_i, 2r_i)| > r^{4/3}$, then call \texttt{OldSpanner} on graph $G[B(v_i, 2r_i)]$. Add the spanner output by \texttt{OldSpanner} to $H$.  Repeat steps 4 and 5 for all $i \in [1, k]$. 
\end{enumerate}
\textbf{Greedy Phase:}

While there exists a pair of vertices $(s, t)$ in $V$ such that $d_H(s, t) > d_G(s, t) + 16\hat{r}$, do the following. Let $\pi$ be a shortest $(s, t)$-path. 
Let $x$ be the vertex in $\pi$ farthest from $s$ such that
for any two vertices $u, w$ in $ \pi(s, x)$, $d_H(u, w) \leq d_G(u, w) + \hat{r}$. Additionally,  let $y$ be the vertex in $\pi$ farthest from $t$ such that for any two vertices $u, w$ in $\pi(y, t)$,   $d_H( u, w) \leq d_G(u, w) + \hat{r}$. Add a shortest $(x, y)$-path to $H$. 

\end{minipage}
}
    \caption{The recursive procedure for the improved spanner upper bounds.}
    
    \label{fig:spanner_upper}
\end{figure}
\paragraph{Bounding the distortion.} Fix  vertices $s, t \in V$.  If $d_H(s, t) \leq d_G(s, t) + 32\hat{r}$, then we are done. Otherwise, vertex pair $(s, t)$ is considered in some round of the greedy phase. Let path $\pi$ and vertices $x, y$ be as defined in the construction. Note that since a shortest $(x, y)$-path is in $H$, $d_H(x, y) = d_G(x, y)$. 
We have the following:
\begin{align*}
    d_H(s, t) & \leq d_H(s, x) + d_H(x, y) + d_H(y, t) \\ 
   & \leq (d_G(s, x) + \hat{r}) + d_G(x, y) + d_G(y, t) + \hat{r}) \\
 &   \leq d_G(s, t) + 2\hat{r}
\end{align*}
Since $\hat{r} = r \cdot n^{c\epsilon}$ for a universal constant $c > 0$, we may obtain our desired distortion  by taking our construction parameter $\epsilon > 0$ to be sufficiently small.
\paragraph{Bounding the size.} 
We begin by bounding the number of edges added to $H$ in the preprocessing phase. Fix an $i \in [1, k]$. If $B(v_i, 2r_i)$ is a small cluster, then in the preprocessing phase we add a shortest path between all vertices $s \in B(v_i, r_i) \cap V'$ and all vertices $t \in B(v_i, 2r_i) \cap V'$ such that $d_G(s, t) \leq r$. Note that with high probability, $|B(v_i, 2r_i) \cap V'| = O(r^{1/3}\log^{-1}n)$. Additionally, observe that since $s \in B(v_i, r_i)$ and $d_G(s, t) \leq r$, it follows that any shortest $(s, t)$-path in $G$ is contained in $G[B(v_i, 2r_i)]$. We now use distance preserver upper bounds to bound the number of edges added in the process. Given a graph $J$ on $n$ vertices and given $p$ demand pairs of vertices in $J$, there exists a subgraph $J' \subseteq J$ on $O(n^{1/2}p)$ edges that exactly preserves the distances between all $p$ pairs of vertices in $J$. Moreover, choosing $J'$ to be the union of any set of $p$ consistent paths between the demand pairs will achieve this bound. (See \cite{CE06} for  details.) Then since we add a set of $p = |B(v_i, 2r_i) \cap V'|^2 = O(r^{2/3}\log^{-2}n)$ consistent paths to $G[B(v_i, 2r_i)]$ and $B(v_i, 2r_i)$ is a small cluster, it follows that $p = O(B(v_i, 2r_i)^{1/2})$, so we add $n^{1/2} p = O(B(v_i, 2r_i))$ edges to $H$. Otherwise, if $B(v_i, 2r_i)$ is a large cluster, then our recursive spanner call contributes $O_{\epsilon}(|B(v_i, 2r_i)|)$ edges to $H$. Finally, by the low overlap property of Lemma \ref{lem:clustering_lem}, we add $O_{\epsilon}(n)$ edges to $H$ in the preprocessing phase. 


To bound the number of edges added in the greedy phase, we again use a path buying argument. As before, we say that vertices $s, t$ in $V$ are \textit{connected} in $H$ if $d_H(s, t) \leq d_G(s, t) + 8\hat{r}$. Each time we add an edge to $H$ in the greedy phase, we will argue that $\Omega(n)$ pairs of vertices in $V$ become connected in $H$ for the first time. Then since there are $O(n^2)$ pairs of vertices in $V$, the greedy phase adds $O(n)$ edges to $H$. Note that the key difference here (compared to the emulator proof) is that we may possibly add many edges to $H$ in each round of the greedy phase since we add entire paths to $H$.

Let $(s, t)$ be a pair of vertices considered in some round of the greedy phase. Let path $\pi$ and vertices $x, y$ be as defined in the construction. We say that paths $\pi(s, x)$ and $\pi(y, t)$ are the prefix and suffix of $\pi$, respectively. Likewise, we call subpath $\pi(x, y)$ the middle of $\pi$. We will define a set $S$ of vertices in $G$ near the middle of $\pi$, as well as sets $T_1$ and $T_2$ of vertices near the prefix and suffix of $\pi$, respectively. Then we will show that after adding edge $(x, y)$ to $H$, every vertex in $S$ either becomes connected in $H$ to every vertex in $T_1$ or to every vertex in $T_2$ for the first time.  

We define $S$, $T_1$, and $T_2$ as follows:
\[
S := \cup_{v \in \pi(x, y)} C(v) \qquad  T_1 := \cup_{v \in \pi(s, x)} C(v) \qquad T_2 := \cup_{v \in \pi(y, t)} C(v)
\]
 We now verify that $S$, $T_1$, and $T_2$ satisfy our desired properties.
 \begin{proposition}
 After path $\pi(x, y)$ is added to $H$, for every vertex $v \in S$, either all pairs of vertices in $\{v\} \times T_1$ or all pairs of vertices in $\{v\} \times T_2$ become connected in $H$ for the first time. 
 \label{prop:new_conn_span}
 \end{proposition}
 \begin{proof}
Fix vertices $s' \in S$, $t_1' \in T_1$, and $t_2' \in T_2$. Let $u, v,$ and $w$ be the vertices in $\pi(x, y)$, $\pi(s, x)$, $\pi(y, t)$ that are closest to $s', t_1',$ and $t_2'$ in $G$, respectively. (See Figure \ref{fig:spanner_drawing} for a visualization.) Note that $d_G(s', u) \leq \hat{r} \log n$, $d_G(t_1', v) \leq \hat{r}/\log n$, and $d_G(t_2', w) \leq \hat{r} / \log n$, by the definition of $S, T_1$, and $T_2$. 
After path $\pi(x, y)$ is added to $H$, pair $(s', t_1')$ is connected in $H$:
\begin{align*}
d_H(s', t_1')  & \leq d_H(s', u) + d_H(u, v) + d_H(v, t_1') \\
& \leq \log n \cdot d_G(s', u) + d_H(u, v) + \log n \cdot d_G(v, t_1') \\
& \leq \hat{r} + d_H(u, x) + d_H(x, v) + \hat{r} \\
& \leq d_H(u, x) + d_G(x, v) + 2\hat{r}  \\
& \leq d_G(u, v) + 3\hat{r} \\
& \leq d_G(u, s') + d_G(s', t_1') + d_G(t_1', v) + 3\hat{r} \\
& \leq d_G(s', t_1') + 5\hat{r}
\end{align*}
where the fifth inequality follows from our choice of $x$. A symmetric argument shows that pair $(s', t_2')$ is also connected in $H$ after $\pi(x, y)$ is added. Now suppose for the sake of contradiction that both pair $(s', t_1')$ and $(s', t_2')$ are connected in $H$ \textit{before} path $\pi(x, y)$ is added. Then we claim that pair $(s, t)$ had how distortion in $H$ before path $\pi(x, y)$ was added:
\begin{align*}
    d_H(s, t) & \leq d_H(s, v) + d_H(v, t_1') + d_H(t_1', t_2') + d_H(t_2', w) + d_H(w, t) \\  
    & \leq (d_G(s, v) + \hat{r}) +  \hat{r} + (d_H(t_1', s') + d_H(s', t_2')) + \hat{r} + (d_G(w, t) + \hat{r}) \\
    & \leq d_G(s, v) + (d_G(t_1', s') + 8\hat{r}) + (d_G(s', t_2') + 8\hat{r}) + d_G(w, t) + 4\hat{r} \\
    & \leq d_G(s, v) + d_G(t_1', v) + d_G(v, u) + d_G(u, s') + d_G(s', u) + d_G(u, w) + d_G(w, t_2') + d_G(w, t) + 20\hat{r} \\
    & \leq d_G(s, t) + 24\hat{r}
\end{align*}
(The final inequality follows from the fact that $\pi$ is a shortest $(s, t)$-path that passes through $v, u$, and $w$ in that order.) This violates our assumption that pair $(s, t)$ was considered in this round of the greedy phase, so we conclude that either pair $(s', t_1')$ or $(s', t_2')$ became connected in $H$ for the first time after path $\pi(x, y)$ was added. 
 \end{proof}
 \begin{figure}[h]
     \centering
     \includegraphics{spanner_drawing.pdf}
     \caption{The solid black line denotes path $\pi$ in $G$. After path $\pi(x, y)$ is added to $H$ in the greedy phase, either pair $(s, t_1')$ or $(s, t_2')$ becomes connected in $H$ for the first time, for all $s \in S$, $t_1' \in T_1$, and $t_2' \in T_2$.  }
     \label{fig:spanner_drawing}
 \end{figure}
Now we need to lower bound $|S|$, $|T_1|$, and $|T_2|$ to complete our upper bound on the number of edges added to $H$ in the greedy phase.
\begin{proposition}
$|T_1| = \Omega(r^{7/3 - 4/3\cdot \alpha}\log n)$ and $|T_2| =\Omega(r^{7/3 - 4/3\cdot \alpha}\log n)$. 
\label{prop:size_t1_t2}
\end{proposition}
\begin{proof}
This proposition will follow from an argument very similar to that of Proposition \ref{prop:s_t_size}.  We will lower bound $|T_1|$; the lower bound for $|T_2|$ follows from a symmetric argument.  
Moreover, instead of lower bounding $|T_1|$ directly, we  find it easier to lower bound the size of a subset $T_1' \subseteq T_1$. We now explicitly construct $T_1'$. We begin the construction by initializing two sets as $U := \emptyset$ and $T_1' := \emptyset$ and setting an integer counter 
$\texttt{err} := 0$. Starting at $s$, we walk through $\pi(s, x)$ as follows. Let $s_1$ be a vertex in $\pi(s, x) \cap V'$ such that $d_G(s, s_1) \leq r$. Note that since we sample vertices in $V$ into $V'$ with probability $\Theta(\log n / r)$, such a vertex $s_1$ will exist with high probability by the Chernoff bound. Add $s_1$ to $U$ and add the vertices in $C(s_1)$ to $S'$. Now, given $s_i$, we let $s_{i+1}$ be a vertex in $\pi(s_i, x) \cap V'$ such that $r/2 \leq d_G(s_i, s_{i+1}) \leq r$. Again by the Chernoff bound, such a vertex $s_{i+1}$ will exist with high probability.
Add vertex $s_{i+1}$ to $U$, and add the vertices in cluster $C(s_{i+1})$ to $S'$. 
If $C(s_i)$ is a large cluster, then we increment $\texttt{err}$ by $+O(|C(s_i)|^{\alpha + \epsilon})$, which corresponds to the distortion of the linear sized spanner of $C(s_i)$ we inserted into $H$ in the preprocessing phase. We proceed in this manner until we add the first vertex $s_{\ell}$ such that $\texttt{err} + O(|C(s_{\ell})|^{\alpha + \epsilon}) > \hat{r} / 2$. (This implies that  $\texttt{err} \leq \hat{r} /2$.) Note that $T_1' = \cup_{s_i \in U}C(s_i)$.

Now we verify that $T_1' \subseteq T_1$, as desired. To prove this, it will suffice to show that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$. Fix an $i \in [1, \ell - 1]$ and suppose that $C(s_i)$ is a small cluster. Then since $s_i$ is in the core of cluster $C(s_i)$ and $d_G(s_i, s_{i+1}) \leq r$, it follows that $s_{i+1} \in C(s_i)$.  Note that in this case, a shortest $(s_i, s_{i+1})$-path is added to $H$ in the preprocessing phase, allowing us to travel from $s_i$ to $s_{i+1}$ in $H$ without incurring any error. Specifically, $d_H(s_i, s_{i+1}) = d_G(s_i, s_{i+1})$.  Otherwise, $C(s_i)$ is a large cluster. In this case, we added a spanner of $G[C(s_i)]$ with additive distortion $+O(|C(s_i)|^{\alpha + \epsilon})$ to $H$ in the preprocessing phase. Note that since $s_i$ is in the core of $C(s_i)$ and $d_G(s_i, s_{i+1}) \leq r$, it follows that any shortest $(s_i, s_{i+1})$-path in $G$ is contained in $G[C(s_i)]$. Consequently, $d_H(s_i, s_{i+1}) \leq d_G(s_i, s_{i+1}) + O(|C(s_i)|^{\alpha + \epsilon})$.
Then by the previous observations, we  conclude that $d_H(s_i, s_j) \leq d_G(s_i, s_j) + \texttt{err}$ for all $i, j \in [1, \ell]$. 
Now let $u, w$ be vertices in $\pi(s, s_{\ell})$ (where $u$ occurs before $w$ in $\pi(s, s_{\ell})$), and let $s_i, s_j$ be the vertices in $\pi(s, s_{\ell}) \cap U$ that are closest to  $u$ and closest to $w$, respectively. Observe that
\begin{align*}
    d_H(u, w) & \leq d_H(u, s_i) + d_H(s_i, s_j) + d_H(s_j, w) \\
    & \leq \log n \cdot d_G(u, s_i) + d_H(s_i, s_j) + \log n \cdot d_G(s_j, w) \\
    & \leq d_G(u, s_i) + d_H(s_i, s_j) + d_G(s_j, w) + 2r\log n \\
    & \leq d_G(u, s_i) + (d_G(s_i, s_j) + \texttt{err}) + d_G(s_j, w) + 2r\log n \\
    & \leq d_G(u, w) + \hat{r}/2 + 2r \log n \\
    & \leq d_G(u, w) + \hat{r}.
\end{align*}
Then by our choice of $x$, it follows that $\pi(s, s_{\ell})$ is a subpath of $\pi(s, x)$, so $T_1' \subseteq T_1$. 

By our construction of $T_1'$, we have the guarantee that $\sum_{i=1}^{\ell} O(|C(s_{i})|^{\alpha + \epsilon}) > \hat{r} / 2$. 
Moreover, we may assume that all clusters $C(s_i)$ are  large clusters, since as noted earlier we can travel through small clusters with zero distortion. This implies that $|C(s_i)| \geq r^{4/3} \log^{-2} n$. 
Now we wish to lower bound the sum $\sum_{i=1}^{\ell} |C(s_i)|$. We may assume that $\alpha + \epsilon < 1$, and so by a convexity argument it can be seen that the sum $\sum_{i=1}^{\ell} |C(s_i)|$ is minimized (while subject to our guaranteed  inequality) when each large cluster has size $r^{4/3} \log^{-2}n$. Let $q$ be the number of large clusters we pass through in $\pi(s, s_{\ell})$.  Then our guarantee becomes  $\sum_{i=1}^{\ell} O(|C(s_{i})|^{\alpha + \epsilon}) = q \cdot (r^{4/3} \log^{-2}n)^{\alpha + \epsilon} > \hat{r} / 2$. Rearranging this inequality gives us that $q > \hat{r} \cdot r^{-4/3\cdot (\alpha + \epsilon)}$. Now note that since $\hat{r} = r \cdot n^{c\epsilon}$ for a sufficiently large constant $c$, we may assume that $\hat{r} \geq r^{1 + 4/3\cdot \epsilon} \log^3 n$ by taking $c > 4/3$. Now putting it all together, we see that
\[
\sum_{i=1}^{\ell}|C(s_i)| \geq q \cdot r^{4/3} \log^{-2} n \geq \frac{\hat{r} \cdot r^{4/3}}{r^{4/3\cdot (\alpha + \epsilon)} \cdot \log^2 n} \geq \Omega(r^{7/3 - 4/3 \cdot \alpha}\log n)
\]

Now we finish the proof by showing that $|T_1'| = |\cup_{i=1}^{\ell} C(s_i)| = \Omega(\sum_{i=1}^{\ell}|C(s_i)|)$. Recall that $d_G(s_i, s_{i+1}) \geq r/2$. Then each vertex $v \in V$ can only occur in $O(1)$ distinct clusters $C(s_i)$, where $s_i \in U$, or else we contradict our assumption that $\pi(s, x)$ is a shortest path in $G$. We conclude that $|\cup_{i=1}^{\ell} C(s_i)| = \Omega(\sum_{i=1}^{\ell}|C(s_i)|)$, so $|T_1| \geq |T_1'| = \Omega(r^{7/3 - 4/3 \cdot \alpha}\log n)$. A symmetric argument establishes the same bound for $|T_2|$.  
% By the coverage property of Lemma \ref{lem:clustering_lem}, we know that every vertex $u_j$ belongs to some cluster core $B(v_{i_j}, r_{i_j})$ for some $i_j \in [1, k]$. Consequently, $u_{j+1} \in B(v_{i_j}, 2r_{i_j})$. In other words,
% consecutive sampled vertices $u_j, u_{j+1}$  in $\pi$ belong to the same cluster $B(v_{i_j}, 2r_{i_j})$.  
% Fix a $j \in [1, \ell - 1]$. 
% If $B(v_{i_j}, 2r_{i_j})$ is a small cluster, then edge $(u_j, u_{j+1})$ is added to $H$ in the preprocessing phase of the construction, allowing us to travel from $u_j$ to $u_{j+1}$ in $H$  without incurring any error. Otherwise, $B(v_{i_j}, 2r_{i_j})$ is a large cluster.  Then we added an emulator of $G[B(v_{i_j}, 2r_{i_j})]$ with additive distortion $+O(|B(v_{i_j}, 2r_{i_j})|^{\alpha + \epsilon})$ to $H$ in the preprocessing phase. Note that since $u_j \in B(v_{i_j}, r_{i_j})$ and $d_G(u_j, u_{j+1}) \leq r$, it follows that any shortest $(u_j, u_{j+1})$-path is contained in $G[B(v_{i_j}, 2r_{i_j})]$. Consequently, $d_H(u_j, u_{j+1}) \leq d_G(u_j, u_{j+1}) +O(|B(v_{i_j}, 2r_{i_j})|^{\alpha + \epsilon})$. Thus we are able to travel from $u_j$ to $u_{j+1}$ in $H$ while incurring a small amount of error proportional to the size of the cluster $B(v_{i_j}, 2r_{i_j})$.  
% We will use the observations in the previous paragraph to verify that $|S| = \Omega(n^{1/2})$. The size of $S$ is constrained by our requirement that for any two vertices $v, w$ in $\pi(s, x)$, $d_H(v, w) \leq d_G(v, w) + \hat{r}$. Let $U' \subseteq U$ be the vertices $u_i$ in $\pi(s, x) \cap U$  such that $C(u_i)$ is a large cluster. Ignoring the 
% To lower bound $|S|$, it will suffice to lower bound $| \cup_{u_i \in U'} C(u_i)|$. 
\end{proof}
Now suppose that $k$ edges are contributed to the size of $H$ when path $\pi(x, y)$ is added to $H$.  We wish to relate $k$ to the size of $S$, in order to bound the total number of edges added in the greedy phase. The following proposition accomplishes this. 
\begin{proposition}
Let $k \geq 0$ be the number of edges added to $H$ when path $\pi(x, y)$ is added to $H$. Then  $|S| = \Omega(r^{2/3}k\log^{-1}n)$.
\label{prop:s_size_span}
\end{proposition}
\begin{proof}
We will begin by defining a list $U$ of nodes $s_1, s_2, \dots, s_{\ell}$ in $\pi(x, y) \cap V'$ in a manner similar to Proposition \ref{prop:size_t1_t2}. Specifically, we define $U$ so that
\begin{enumerate}
    \item $s_i$ occurs before $s_j$ in $\pi(x, y)$ if $i < j$
    \item $r/2 \leq d_G(s_i, s_{i+1}) \leq r$ for $i \in [1, \ell - 1]$
    \item $d_G(s, s_1) \leq r$ and $d_G(s_{\ell}, t) \leq r$.
\end{enumerate}
Recall that by the discussion in Proposition \ref{prop:size_t1_t2}, if $C(s_i)$ is a small cluster, then we add a shortest $(s_i, s_j)$-path $\pi'$ to $H$ in the preprocessing phase. Then since we chose path $\pi(x, y)$ to be consistent, it follows that $\pi(x, y)$ has $\pi'$ as a subpath, so we add zero edges in this subpath of $\pi(x, y)$. Otherwise, if $C(s_i)$ is a large cluster, we must add a consistent shortest $(s_i, s_j)$-path to $H$. We note that since $s_i$ is in the core of $C(s_i)$, this path will be contained entirely in $G[C(s_i)]$. Since this path is consistent, we can bound the amortized number of edges added to $H$ in $C(s_i)$ using distance preserver upper bounds. As discussed earlier, distance preserver bounds imply that the average path length of the consistent paths added to $H[C(s_i)]$ in the greedy phase will be $O(|C(s_i)|^{1/2})$. Then on average $O(|C(s_i)|^{1/2})$ edges will be added to $H$ to cover the subpath $\pi(s_i, s_j)$ of $\pi(x, y)$. Moreover, since $C(s_i) \subseteq S$, cluster $C(s_i)$ will contribute $\Omega(|C(s_i)|)$ vertices to $S$. We may assume that all clusters $C(s_i)$ are large clusters, since small clusters have zero distortion.
It follows that $|C(s_i)| = \Omega(r^{4/3}\log^{-2} n)$. 
We have the guarantee that $\sum_{i=1}^{\ell}O(|C(s_i)|^{1/2}) = k$ and we wish to lower bound $|S| \geq \sum_{i=1}^{\ell}|C(s_i)|$. By the same argument as in Proposition \ref{prop:size_t1_t2}, the sum $\sum_{i=1}^{\ell}|C(s_i)|$ is minimized subject to our constraint when $|C(s_i)| = r^{4/3}\log^{-2}n$ for all $i \in [1, \ell]$. In this case,  
\[
\sum_{i=1}^{\ell}|C(s_i)| \geq \ell \cdot  r^{4/3}\log^{-2}n = \Theta(k \cdot r^{2/3} \log^{-1}n)
\]
where the equality follows from the fact that $k  =  \Theta(\ell \cdot r^{2/3} \log^{-1}n)$. Then by the same argument as in Proposition \ref{prop:size_t1_t2},  $|S| \geq |\cup_{i=1}^{\ell}C(s_i)| = \Omega(\sum_{i=1}^{\ell}|C(s_i)|)$, so we conclude that $|S| = \Omega(k \cdot r^{2/3} \log^{-1} n)$ as desired. 
\end{proof}
By Proposition \ref{prop:new_conn_span}, after $\pi(x, y)$ is added to $H$, $\Omega(\min\{|S \times T_1|, |S\times T_2|\})$ pairs of vertices become connected in $H$ for the first time. If $k$ edges are added to $H$ in this round of the greedy phase, then by Propositions \ref{prop:size_t1_t2} and \ref{prop:s_size_span}, 
\[
\min\{|S \times T_1|, |S\times T_2|\}  = kr^{3 - 4/3 \cdot \alpha} = \Omega(kn).
\]
where the final inequality follows from our choice of $r = n^{1/(3 - 4/3 \cdot \alpha)}$.  Then since  we connect $\Omega(n)$ new pairs of vertices in $V$ for each edge added to $H$, we conclude that $O(n)$ edges are added to $H$ in the greedy phase. At most $O_{\epsilon}(n)$ edges are added to $H$ overall.
\end{proof}




% Now we can repeatedly apply Lemma \ref{lem:emu_recursion} to obtain our improved emulator bounds. We choose our initial emulator to be the additive emulator of \cite{BV15} with distortion $+O(n^{1/3})$ and  $\widetilde{O}(n)$ edges. Then after one application of  \ref{lem:emu_recursion}, we obtain an additive emulator with $O_{\epsilon}(n)$ edges and distortion $+O(n^{1/(6 - 4/3) + \epsilon}) = +O(n^{3/14 + \epsilon})$. More generally, after $i$ applications of Lemma \ref{lem:emu_recursion}, we obtain an additive emulator with $O_{\epsilon}(n)$ edges and distortion $+O(n^{a_i + \epsilon})$, where $a_i$ is defined by the recurrence relation $a_0 = 1/3$, $a_{i+1} = 1/(6-4a_i)$. This recurrence relation converges quickly to $\frac{1}{3 + \sqrt{5}} \approx 0.191$.

As with our emulator upper bound, we can repeatedly apply Lemma  \ref{lem:spanner_rec} to obtain improved spanner upper bounds. We choose our initial bound to be the additive spanner of \cite{BV16} with distortion $+O(n^{3/7 + \epsilon})$ and size $O_{\epsilon}(n)$. After $i$ applications of Lemma \ref{lem:spanner_rec}, we obtain a spanner construction with $O_{\epsilon}(n)$ edges and $+O(n^{a_i + \epsilon})$ distortion, where $a_i$ is defined by the recurrence relation $a_0 = 3/7$, $a_{i+1} = 1/(3 - 4/3\cdot a_i)$. The value of $a_i$ converges quickly to the fixed point $\frac{9 - \sqrt{33}}{8} \approx 0.407$. 


\begin{theorem}
For every $n$-node graph $G = (V, E)$ and every $\epsilon > 0$, there exists a spanner $H \subseteq G$ on $O_{\epsilon}(n)$ edges with distortion $+O(n^{\frac{9 - \sqrt{33}}{8} + \epsilon})$.  
\end{theorem}


